Probing Anomalous Higgs Boson Couplings at Colliders

In this thesis, our main focus is on the $HHH$ and $VVHH$ couplings which are loosely bound. The $HHH$ coupling will determine the shape the Higgs potential and $VVHH$ couplings will tell us how the gauge bosons are coupled to the Higgs fields. We consider a few processes of Higgs boson production and decay to study these couplings. We calculate one-loop QCD and electroweak correction for these processes. In this thesis, we discuss spinor helicity formalism, which has been used in computing Feynman amplitudes for QCD and electroweak correction to these processes. We discuss one-loop Feynman integrals and one-loop electroweak renormalization and Catani-Seymour dipole subtraction scheme in this thesis. We compute all possible self-energy contributions at one-loop for electroweak renormalization. In this thesis, in the first work, we consider the process $b\bar{b}\rightarrow W^+W^-H$. Due to the non-negligible coupling of the Higgs boson with the bottom quarks, there is a dependence on the $WWHH$ coupling in this process. We find that the corrections to the final state with the longitudinally polarized $W$ bosons are large. In the second work, we study one-loop electroweak correction to $H\rightarrow \nu_e\bar{\nu_e}\nu_\mu\bar{\nu_\mu}$. We discuss $\gamma^5$-anomaly, complex mass scheme and input parameter schemes which are relevant for one-loop electroweak correction. The corrections depend on the $HHH$ and $ZZHH$ couplings. We investigate this dependence in $\kappa$-framework. In the third work, we study one-loop electroweak correction to the $H\rightarrow e^+e^-\mu^+\mu^-$ process. The corrections depend on $HHH$ and $ZZHH$ couplings. We observe the same behavior in the relative change of the decay width for this process as the process $H\rightarrow \nu_e\bar{\nu_e}\nu_\mu\bar{\nu_\mu}$ when we vary $HHH$ and $ZZHH$ couplings.

==> UV_ol_ren/uv_ol_ren_old.tex <==
\chapter{Renormalization at one loop}
\label{chap_ren_ol}
%  
  In this chapter, we will discuss about the one loop Feynman integrals that appear in the one loop diagram for a quantum field theoretical scattering and decay process. We will see that these integrals are divergent at large loop momenta ($\Lambda\rightarrow \infty$) regime. 
   This type of divergence is called \textit{ultraviolet} (UV) divergence. The standard model is the completely renormalizable theory. In standard model the divergences appear at any order can be absorbed by the bare parameters in the standard model.
   The renormalization perturbation theory tells us how the bare parameters can be written in terms of renormalized parameters and corresponding counterterms. We will discuss about one loop renormalization for QCD and EW in the following sections.
   We adopt the on-shell renormalization scheme for massive particles and $\overline{\text{MS}}$ scheme for massless particles.
   %
\section{One loop integrals}
\label{sec_ren_ol_int}
%
A general one loop integral in $D$ dimension with $N$ number of propagator factor in the denominator and $P$ number of loop momenta in the numerator can be written as 
%
\begin{align}
 T^{(N)}_{\mu_1...\mu_P}(p_0,...,p_{N-1},m_0,...,m_{N-1})=\frac{(2\pi\mu)^{(4-D)}}{i\pi^2}\int d^Dq\frac{q_{\mu_1}...q_{\mu_P}}{N_0...N_{N-1}}\:,
 \label{equ_ren_ol_int}
 \end{align}
%
  with the denominator factors
%
 \begin{align}
 N_0=q^2-m_0^2+i\epsilon\:,\quad D_i=(q+p_i)^2-m_i^2+i\epsilon\:,\quad i=1,...,N-1\:.
 \end{align}
%
  These denominators originate from the propagators in the Feynman diagram. The schematic diagram for one loop integral given in Eq.~\ref{equ_ren_ol_int}, has been shown in Fig.~\ref{fig_ren_ol_gnrc}. The loop momenta for $i^{\text{th}}$ internal leg is $q+p_i$ and the external momenta are
  %
  \begin{align}
   p_{0i}=p_i\quad {\text{and}}\quad p_{ij}=p_i-p_j.
  \end{align}    
  %
\begin{figure}[h!]
 \begin{center}
\includegraphics [angle=0,width=0.4\linewidth]{./one_loop/figures/one_loop_generic.eps}\\
	\caption{Generic one loop $N$-point integral with loop and external momenta.}
	\label{fig_ren_ol_gnrc}
	\end{center}
\end{figure}
  %
  Conventionally, the integral $T^N$ is denoted by alphabets with the $N$ value as $T^1\equiv A$, $T^2\equiv B$, ... and the scalar integrals are denoted by $A_0$, $B_0$, $C_0$, ... . Traditionally, $A$, $B$, $C$, $D$, ... type integrals are called tadpole, bubble, triangle, box, ... type integrals respectively.
  There are several reduction techniques [ref,PV,OV] which help to reduce tensor integral into scalar integrals. The basic property of these reductions is that any integral $T^N$ can be written as a linear combination of one loop scalar integrals and a finite remnant $\mathcal{R}$ of dimensional regularization procedure. This can be expressed as
  %
  \begin{align}
  T^N=c_{4;j}T^4_{0;j}+c_{3;j}T^3_{0;j}+c_{2;j}T^2_{0;j}+c_{1;j}T^1_{0;j}+\mathcal{R}+\mathcal{O}(D-4)\:.
  \label{equ_ren_Tn_decmp}
  \end{align}
  %
  The coefficient $c_{N;j}\:(N=1,...,4)$ in Eq.~\ref{equ_ren_Tn_decmp} are evaluated in $D=4$ dimension i.e, they do not depend on $\epsilon$. They are function of external momenta, masses and the different scalar integrals.
  The $T^N_{0;j}\:(N=0,...,4)$ denote the one loop scalar integral of type $j$. The type $j$ specifies the external momenta that specify the denominators for corresponding scalar integral. This decomposition originates from the Lorentz invariance of decomposition of tensor structure to invariant form factors and the four dimensional nature of space-time which allows the decomposition of higher scalar integrals to sum of box scalar integrals.
  The explicit Lorentz decomposition for bubble tensor integrals can be written as 
  \begin{align}
  T^2_{\mu}\equiv B_\mu= {p_1}_\mu\:B_1\:,\quad T^2_{\mu\nu}\equiv B_{\mu\nu}=g_{\mu\nu}\:B_{00}+{p_1}_\mu {p_1}_\nu\:B_{11}\:.  
  \end{align}
  %
  In similar way, one can write the decomposition of other tensor integrals too[deneree][ellis].
  
  The integral given in Eq.~\ref{equ_ren_ol_int} are UV divergent with the condition $P+D-2N \geq 0$. The UV divergences are regularized in dimensional regularization in which the one loop integrals have been evaluated in $D$ dimension. 
  The UV divergence comes only from tadpole and bubble scalar integrals. In cut-off regularization, we can easily see the divergences in $D=4$ dimension as below
  \begin{align}
  A_0\sim\int^\Lambda \frac{d^4q}{N_0}\sim\int^\Lambda \frac{d^4q}{q^2}\sim \Lambda^0\:,\quad B_0\sim\int^\Lambda \frac{d^4q}{N_0N_1}\sim\int^\Lambda \frac{d^4q}{q^2.q^2}\sim \Lambda^2\:.
  \label{equ_ren_a0_b0_uv}
  \end{align}
  %
  In Eq.~\ref{equ_ren_a0_b0_uv}, the $A_0$ is logarithmic and $B_0$ is quadratic divergent. In dimension regularization these divergences appear as $\frac{1}{\epsilon}$ poles. The UV poles for these two scalar integrals in dimensional regularization are
  \begin{align}
  A_0(m)\Big\vert_{UV} = -2m^2\:\frac{1}{D-4}\:\quad {\text{and}}\quad B_0(p_1,m_0,m_1)\Big\vert_{UV}=-2\:\frac{1}{D-4}\:.
  \end{align}
  %
  One can remove the UV divergences by renormalizing the bare parameters and the fields for a given renormalizable theory. 
%
%\section{QCD renormalization at one loop}
%\label{sec_ren_qcd_ol_ren}
%
\section{EW renormalization at one loop}
\label{sec_ren_ew_ol_ren}
%
 The parameters in standard model have to be extracted with the experiments. The parameters are coupling, masses. The tree level physical observables can be calculated with these parameters and they have direct relations with the experiments.
 This scenario become problematic in higher order correction. As we have seen that the higher order corrections can be UV divergent. In a renormalizable theory, these UV divergences can be dropped and one  can predict the physical observables with the higher order accuracy.
 The procedure of renormalization for a renormalizable theory involves the redifination of bare SM parameters and fields in terms of renormalized parameters and fields. The renormalized parameters are related to predict the physical observables whereas the field renormalization make Green functions finite.
 The heavy particles mass is known from experiments, so on-shell renormalization scheme is a good choice for the renormalization  associated with heavy particle. The particles whose masses are not known properly the $\overline{\text{MS}}$ renormalization scheme will be convenient for them.
 There are many independent parameters sets with which one can proceed renormalization. We choose the parameter set: $e$, $M_W$, $M_Z$, $M_H$, and $m_f$. Here $e$ is the electric charge, $M_W$, $M_Z$, $M_H$, and $m_f$ are the masses of $W$, $Z$, $H$ boson and fermions respectively.
  We take the quark mixing CKM matrix [] $V_{CKM}$ as diagonal, so no renormalization is needed for $V_{CKM}$. We adopt on-shell renormalization scheme for electroweak standard model. Here we will only discuss about the certain renormalization which is relevant for  the process discussed in Chap.~\ref{chap_h24nu} and~\ref{chap_h22e2m}.
  
  We express the bare parameters in terms of renormalized parameters and corresponding counterterm as below
  \begin{align}
  e_0=(1+\delta Z_e)e\:,\quad M^2_{W,0}=M^2_{W}+\delta M^2_W\:,\quad
  M^2_{Z,0}=M^2_Z+\delta M_Z^2\:.
  \label{equ_ren_ren_para}
  \end{align}
 %
 As we have discussed that the fields are also needed to renormalize. We write the similar expressions like in Eq.~\ref{equ_ren_ren_para} for the fields renormalization as below
 \begin{align}
 Z_0=(1+\frac{1}{2}\delta Z_{ZZ})\: Z+\frac{1}{2}\delta Z_{ZA}\; A\:,&\quad A_0=(1+\frac{1}{2}\delta Z_{AA})\: A+\frac{1}{2}\delta Z_{AZ}\: Z\:,\nonumber \\
W_0^\pm=(1+\frac{1}{2}\delta Z_W)\: W^\pm\:,&\quad\:H_0=(1+\frac{1}{2}\delta Z_H)\: H\:,\nonumber \\
f_{i,0}^L=(\delta_{ij}+\frac{1}{2}\delta Z_{ij}^{f,L})\: f_j^L\:,&\quad f_{i,0}^R=(\delta_{ij}+\frac{1}{2}\delta Z_{ij}^{f,R})\: f_j^R\:.
\label{equ_ren_ren_wf}
 \end{align}
 %
 We denote bare quantities by the '$0$' and the renormalized quantities in normal fashion in Eq.~\ref{equ_ren_ren_para},~\ref{equ_ren_ren_wf}. The $\delta Z$s and $\delta M$s in Eq.~\ref{equ_ren_ren_para},~\ref{equ_ren_ren_wf} are the renormalization constants.
 In renormalization perturbation theory with the expansion $Z=1+\delta Z$, the bare Lagrangian $\mathcal{L}_0$  can be written as
 \begin{align}
 \mathcal{L}_0=\mathcal{L}+\delta \mathcal{L}\:,
 \end{align}
 %
 where the $\mathcal{L}$ is the renormalized Lagrangian which depends on renormalized parameters and fields; and $\delta \mathcal{L}$ is the counterterm.
 One can set up the Feynman rules for counterterms from $\delta \mathcal{L}$ and all possible counterterm diagrams for a given process.
 %
 The renormalization constants given in Eq.~\ref{equ_ren_ren_para},~\ref{equ_ren_ren_wf} can determined by the suitable on-shell renormalization conditions[]. Following the Ref[], we write the explicit expression form of the renormalization constants as below
%
\begin{align}
\delta M_W^2={\text {Re}}\:\Sigma ^W_T(M_W^2)\:,\quad& \delta Z_W=-{\text{Re}}\frac{\partial}{\partial k^2}\Sigma^W_T(k^2)\bigg |_{k^2=M_W^2}\:,\nonumber\\
\delta M_Z^2={\text {Re}}\:\Sigma ^{ZZ}_T(M_Z^2)\:,\quad& \delta Z_{ZZ}=-{\text{Re}}\frac{\partial}{\partial k^2}\Sigma^{ZZ}_T(k^2)\bigg |_{k^2=M_Z^2}\:,\nonumber\\
\delta Z_{ZA}=2\frac{\Sigma^{AZ}_T(0)}{M_Z^2},\quad& \delta Z_{AA}=-\frac{\partial}{\partial k^2}\Sigma^{AA}_T(k^2)\bigg |_{k^2=0}\:,\quad\nonumber\\
\delta Z_e=-\frac{1}{2}\delta Z_{AA}-\frac{s_W}{c_W}\frac{1}{2}\delta Z_{ZA}\:,\quad&\delta Z_{H}=-{\text{Re}}\frac{\partial}{\partial k^2}\Sigma^H(k^2)\bigg |_{k^2=M_H^2}\:,\nonumber\\
\delta Z_{ii}^{f,L}=-{\text {Re}}\:\Sigma_{ii}^{f,L}(m_{f,i}^2)-m_{f,i}^2\frac{\partial}{\partial k^2}{\text {Re}}&\Big[\Sigma_{ii}^{f,L}(k^2)+\Sigma_{ii}^{f,R}(k^2)+2\Sigma_{ii}^{f,S}(k^2)\Big]\bigg |_{k^2=m_{f,i}^2}\:,\nonumber\\
\delta Z_{ii}^{f,R}=-{\text {Re}}\:\Sigma_{ii}^{f,R}(m_{f,i}^2)-m_{f,i}^2\frac{\partial}{\partial k^2}{\text {Re}}&\Big[\Sigma_{ii}^{f,L}(k^2)+\Sigma_{ii}^{f,R}(k^2)+2\Sigma_{ii}^{f,S}(k^2)\Big]\bigg |_{k^2=m_{f,i}^2}\:.
\label{equ_ren_ren_cnst}
\end{align}
%
 The $\sum$ in Eq.~\ref{equ_ren_ren_cnst} are the self energies for different propagators. In the next section, we have wrote down the explicit expressions for various self energies which are relevant for the process given in Chap.~\ref{chap_h24nu},~\ref{chap_h22e2m}.
 %
 %
 \subsection{Self energies}
 \label{equ_ren_slf_enrg}
 %
 We denote Gold-stone bosons by $G^{\pm,0}$ and ghost fields by $\eta^{\pm,Z,\gamma}$. All fermions loop diagrams have been shown with one generic diagram with the fermion line $f$. The momentum $p$ is the incoming and outgoing momenta for all self energy diagrams in this section. We drop $\frac{\alpha}{2\pi}$ factor from each self energy as it is a common factor all.
 \subsubsection{Photon self energy :}
 \label{equ_ren_gam_se} 
   %
\begin{figure}[h!]
 \begin{center}
\includegraphics [angle=0,width=0.7\linewidth]{./one_loop/figures/gam_gam.eps}\\
	\caption{Photon self energy diagrams at one loop.}
	\label{fig_ren_self_gam_gam}
	\end{center}
\end{figure}
%
 We have listed the photon self energy diagrams in Fig.~\ref{fig_ren_self_gam_gam}. The contribution for the self energy diagram of photon from each sub diagrams in Fig.~\ref{fig_ren_self_gam_gam} are listed below 
 \begin{align}
 \Sigma_T^{AA}(p^2)=&\quad 2\Big[4A_0(M_W^2)-2M_W^2C_I^R\Big]\quad\quad\quad\quad\quad\quad\quad\quad\quad\quad\quad\quad\quad
 ....\:({\text{dia. a and b}})\nonumber\\
 &+2B_{00}(p^2,M_W^2,M_W^2)\quad\quad\quad\quad\quad\quad\quad\quad\quad\quad\quad\quad
 \quad\quad\quad ....\:({\text{dia. c and d}})\nonumber\\
 &-4B_{00}(p^2,M_W^2,M_W^2)\quad\quad\quad\quad\quad\quad\quad\quad\quad\quad\quad
 \quad\quad\quad\quad ....\: ({\text{dia. e}})\nonumber\\
 &-2M_W^2B_{0}(p^2,M_W^2,M_W^2)\quad\quad\quad\quad\quad\quad\quad\quad\quad\quad\quad\quad\quad
 \:\: .... \:({\text{dia. f and g}})\nonumber\\
 &+\Big[-10B_{00}(p^2,M_W^2,M_W^2)-2A_0(M_W^2)-(2M_W^2+4p^2).\nonumber\\
 &\quad\quad\quad\quad B_0(p^2,M_W^2,M_W^2)+(4M_W^2-\frac{p^2}{6})C_I^R\Big]
 \quad\quad\quad\quad\:\:\: ....\:({\text{dia. h}})\nonumber\\
 &+4\Big[\frac{1}{3}(p^2+2m_f^2)B_{0}(p^2,m_f^2,m_f^2)-\frac{p^2}{9}\nonumber\\
&\quad\quad\quad -\frac{2}{3}m_f^2 B_0(0,m_f^2,m_f^2)\Big]
 \quad\quad\quad\quad\quad\quad\quad\quad\quad\quad\quad\quad ....\:({\text{dia. i}})\nonumber\\
 \end{align}
 %
 %
 %
 \subsubsection{$\gamma\text{-} Z$ boson self energy :}
 \label{equ_ren_self_a_z} 
   \begin{figure}[h!]
 \begin{center}
\includegraphics [angle=0,width=0.7\linewidth]{./one_loop/figures/gam_z.eps}\\
	\caption{$\gamma{\text{-}Z}$ boson self energy diagrams at one loop.}
	\label{fig_ren_self_gam_z}
	\end{center}
\end{figure}
%
 We have listed the $\gamma\text{-}Z$ boson self energy diagrams in Fig.~\ref{fig_ren_self_gam_z}. The contributions for the $\gamma\text{-}Z$ boson self energy diagram from each sub diagrams in Fig.~\ref{fig_ren_self_gam_z} are listed below 
 \begin{align}
 \Sigma_T^{AZ}(p^2)=&-\frac{(2c_W^2-1)}{s_Wc_W}\:A_0(M_W^2)\quad\quad\quad\quad\quad\quad\quad\quad\quad\quad\quad\quad
 \quad\quad\quad\:\:
 ....\:({\text{dia. a}})\nonumber\\
 &-2\frac{c_W}{s_W} (3A_0(M_W^2)-2M_W^2C_I^R)\quad\quad\quad\quad\quad\quad\quad\quad\quad\quad\quad
 \quad ....\:({\text{dia. b}})\nonumber\\
 &+2\frac{(2c_W^2-1)}{s_Wc_W}\:B_{00}(p^2,M_W^2,M_W^2)\quad\quad\quad\quad\quad\quad\quad\quad\quad\quad
 \quad ....\: ({\text{dia. c}})\nonumber\\
 &-2\frac{c_W}{s_W}\:B_{00}(p^2,M_W^2,M_W^2)\quad\quad\quad\quad\quad\quad\quad\quad\quad\quad\quad\quad\quad \quad.... \:({\text{dia. d and e}})\nonumber\\
 &+2\frac{s_W}{c_W}\:B_{0}(p^2,M_W^2,M_W^2)\quad\quad\quad\quad\quad\quad\quad\quad\quad\quad\quad\quad
 \quad\quad\quad .... \:({\text{dia. f and g}})\nonumber\\
 &-\frac{c_W}{s_W}\Big[-10B_{00}(p^2,M_W^2,M_W^2)-2A_0(M_W^2)-(2M_W^2+4p^2).\nonumber\\
 &\quad\quad\quad\quad B_0(p^2,M_W^2,M_W^2)+(4M_W^2-\frac{p^2}{6})C_I^R\Big]
 \quad\quad\quad\quad\quad\quad ....\:({\text{dia. h}})\nonumber\\
 &-\frac{2}{3}Q_f(g^+_f+g^-_f)\Big[(p^2+2m_f^2)B_{0}(p^2,m_f^2,m_f^2)-\frac{p^2}{3}\nonumber\\
&\quad\quad\quad -2m_f^2 B_0(0,m_f^2,m_f^2)\Big]
 \quad\quad\quad\quad\quad\quad\quad\quad\quad\quad\quad\quad
 \quad\:\: ....\:({\text{dia. i}})\nonumber\\
 \end{align}
 %
 \subsubsection{$Z$ boson self energy :}
 \label{equ_ren_self_zz} 
   \begin{figure}[h!]
 \begin{center}
\includegraphics [angle=0,width=0.7\linewidth]{./one_loop/figures/z_z_self.eps}\\
	\caption{$Z$ boson self energy diagrams at one loop.}
	\label{fig_ren_self_zz}
	\end{center}
\end{figure}
%
 We have listed the $Z$ boson self energy diagrams in Fig.~\ref{fig_ren_self_zz}. The contributions for the $Z$ boson self energy diagram from each sub diagrams in Fig.~\ref{fig_ren_self_zz} are listed below 
 \begin{align}
 \Sigma_T^{ZZ}(p^2)=&\quad\frac{1}{4s_W^2c_W^2}\:A_0(M_H^2)\quad\quad\quad\quad\quad\quad\quad\quad\quad\quad\quad\quad
 \quad\quad\quad\quad\quad
 ....\:({\text{dia. a}})\nonumber\\
 &+\frac{1}{4s_W^2c_W^2}\:A_0(M_Z^2)\quad\quad\quad\quad\quad\quad\quad\quad\quad\quad\quad\quad\quad
 \quad\quad\quad\quad ....\:({\text{dia. b}})\nonumber\\
 &+\frac{(2c_W^2-1)^2}{2s_W^2c_W^2}\:A_0(M_W^2)\quad\quad\quad\quad\quad\quad\quad\quad\quad\quad\quad\quad
 \quad\quad\quad\: ....\: ({\text{dia. c}})\nonumber\\
 &+2\frac{c_W^2}{s_W^2}\:(3A_0(M_W^2)-2M_W^2C_I^R)\quad\quad\quad\quad\quad\quad\quad\quad\quad\quad\quad\quad.... \:({\text{dia. d}})\nonumber\\
 &-\frac{1}{s_W^2c_W^2}\:B_{00}(p^2,M_Z^2,M_H^2)\quad\quad\quad\quad\quad\quad\quad\quad\quad\quad\quad
 \quad\quad\quad .... \:({\text{dia. e}})\nonumber\\
  &-\frac{(2c_W^2-1)^2}{s_W^2c_W^2}\:B_{00}(p^2,M_W^2,M_W^2)\quad\quad\quad\quad\quad\quad\quad\quad\quad
 \quad\quad\:\:\: .... \:({\text{dia. f}})\nonumber\\
 &+2\frac{c_W^2}{s_W^2}\:B_{00}(p^2,M_W^2,M_W^2)\quad\quad\quad\quad\quad\quad\quad\quad\quad\quad\quad
 \quad\quad\quad\:\:\: .... \:({\text{dia. g and h}})\nonumber\\
 &+\frac{M_Z^2}{s_W^2c_W^2}\:B_{0}(p^2,M_Z^2,M_H^2)\quad\quad\quad\quad\quad\quad\quad\quad\quad\quad\quad\quad
 \quad\quad\:\:\: .... \:({\text{dia. i}})\nonumber\\
 &+2M_Z^2s_W^2\:B_{0}(p^2,M_W^2,M_W^2)\quad\quad\quad\quad\quad\quad\quad\quad\quad\quad\quad
 \quad\quad\quad .... \:({\text{dia. j and k}})\nonumber\\
 &-\frac{c_W^2}{s_W^2}\Big[10B_{00}(p^2,M_W^2,M_W^2)+2A_0(M_W^2)+(2M_W^2\nonumber\\
 &\quad\quad\quad +4p^2)B_0(p^2,M_W^2,M_W^2)+(4M_W^2-\frac{p^2}{6})C_I^R\Big]
 \quad\quad\quad\quad\: ....\:({\text{dia. l}})\nonumber\\
 &-\Big[\frac{2}{3}((g^+_f)^2+(g^-_f)^2)\Big\{-(p^2+2m_f^2)B_{0}(p^2,m_f^2,m_f^2)+\frac{p^2}{3}\nonumber\\
&\quad\quad +2m_f^2 B_0(0,m_f^2,m_f^2)\Big\}+\frac{1}{2s_W^2c_W^2}m_f^2B_0(p^2,m_f^2,m_f^2)\Big]
 \quad\:\: ....\:({\text{dia. m}})\nonumber\\
 \end{align}
 %
  \subsubsection{$W$ boson self energy :}
 \label{equ_ren_self_ww} 
 We have listed the $W$ boson self energy diagrams in Fig.~\ref{fig_ren_self_ww}. The contributions for the $\gamma\text{-}Z$ boson self energy diagram from each sub diagrams in Fig.~\ref{fig_ren_self_ww} are listed below
 \newpage
   \begin{figure}[h!]
 \begin{center}
\includegraphics [angle=0,width=0.7\linewidth]{./one_loop/figures/w_w_self.eps}\\
	\caption{$\gamma{\text{-}Z}$ boson self energy diagrams at one loop.}
	\label{fig_ren_self_ww}
	\end{center}
\end{figure}
% 
 \begin{align}
 \Sigma_T^{W}(p^2)=&\quad\frac{1}{4s_W^2}\:A_0(M_H^2)\quad\quad\quad\quad\quad\quad\quad\quad\quad\quad\quad\quad\quad
 \quad\quad\quad\quad\quad\:
 ....\:({\text{dia. a}})\nonumber\\
 &+\frac{1}{4s_W^2}\:A_0(M_Z^2)\quad\quad\quad\quad\quad\quad\quad\quad\quad\quad\quad\quad\quad
 \quad\quad\quad\quad\quad\: ....\:({\text{dia. b}})\nonumber\\
 &+\frac{1}{2s_W^2}\:A_0(M_W^2)\quad\quad\quad\quad\quad\quad\quad\quad\quad\quad\quad\quad
 \quad\quad\quad\quad\quad\quad ....\: ({\text{dia. c}})\nonumber\\
 &+0\quad\quad\quad\quad\quad\quad\quad\quad
 \quad\quad\quad\quad\quad\quad\quad\quad
 \quad\quad\quad\quad\quad\quad\quad\:\:\: ....\: ({\text{dia. d}})\nonumber\\
 &+\frac{c_W^2}{s_W^2}\:(3A_0(M_Z^2)-2M_Z^2C_I^R)\quad\quad\quad\quad\quad\quad\quad\quad\quad\quad\quad
 \quad\quad.... \:({\text{dia. e}})\nonumber\\
 &+\frac{1}{s_W^2}\:(3A_0(M_W^2)-2M_W^2C_I^R)\quad\quad\quad\quad\quad\quad\quad\quad\quad\quad\quad
 \quad\:\: .... \:({\text{dia. f}})\nonumber\\
 &-\frac{1}{s_W^2}\:B_{00}(p^2,M_H^2,M_W^2)\quad\quad\quad\quad\quad\quad\quad\quad\quad\quad\quad
 \quad\quad\quad\:\:\:\: .... \:({\text{dia. g}})\nonumber\\
 &-\frac{1}{s_W^2}\:B_{00}(p^2,M_Z^2,M_W^2)\quad\quad\quad\quad\quad\quad\quad\quad\quad\quad\quad
 \quad\quad\quad\:\:\:\: .... \:({\text{dia. h}})\nonumber\\
  &+2B_{00}(p^2,M_W^2,0)\quad\quad\quad\quad\quad\quad\quad\quad
  \quad\quad\quad\quad\quad\quad\quad
 \quad\quad\:\: .... \:({\text{dia. i and j}})\nonumber\\
 &+2\frac{c_W^2}{s_W^2}\:B_{00}(p^2,M_W^2,M_W^2)\quad\quad\quad\quad\quad\quad\quad\quad\quad\quad\quad
 \quad\quad\quad\:\: .... \:({\text{dia. k and l}})\nonumber\\
 &+M_W^2\:B_{0}(p^2,0,M_W^2)\quad\quad\quad\quad\quad\quad\quad\quad\quad\quad\quad\quad\quad
 \quad\quad\quad\:\: .... \:({\text{dia. m}})\nonumber\\
 &+M_Z^2s_W^2\:B_{0}(p^2,M_Z^2,M_W^2)\quad\quad\quad\quad\quad\quad\quad\quad\quad\quad\quad
 \quad\quad\quad\: .... \:({\text{dia. n}})\nonumber\\
 &+\frac{M_W^2}{s_W^2}\:B_{0}(p^2,M_H^2,M_W^2)\quad\quad\quad\quad\quad\quad\quad\quad\quad\quad\quad
 \quad\quad\quad\quad .... \:({\text{dia. o}})\nonumber\\
 &-\Big[10B_{00}(p^2,0,M_W^2)+2A_0(M_W^2)+2p^2B_1(p^2,0,M_W^2)\nonumber\\
 &\quad\quad\quad +5p^2B_0(p^2,0,M_W^2)-2(M_W^2-\frac{p^2}{3})C_I^R\Big]
 \quad\quad\quad\quad\quad\:\:\: ....\:({\text{dia. p}})\nonumber\\
 &-\frac{c_W^2}{s_W^2}\Big[10B_{00}(p^2,M_W^2,M_Z^2)+2A_0(M_W^2)\nonumber\\
 &\quad\quad\quad +(2M_Z^2+3p^2)B_0(p^2,M_W^2,M_Z^2)-2P_1^2B_1(p^2,0,M_W^2)\nonumber\\
 &\quad\quad\quad -\frac{2}{3}(3M_W^2+3M_Z^2-p^2)C_I^R\Big]
 \quad\quad\quad\quad\quad\quad\quad\quad
 \quad\quad\:\:\: ....\:({\text{dia. q}})\nonumber\\
 &-\frac{1}{3s_W^2}\Big[-\Big(p^2-\frac{m_f^2+m_{f^\prime}^2}{2}\Big)B_{0}(p^2,m_f^2,m_{f^\prime}^2)+\frac{p^2}{3}\nonumber\\
&\quad\quad +\Big(m_f^2 B_0(0,m_f^2,m_f^2)+m_{f^\prime}^2 B_0(0,m_{f^\prime}^2,m_{f^\prime}^2)\Big)\nonumber\\
&+\frac{(m_f^2-m_{f^\prime}^2)}{2p^2}\Big(B_0(p^2,m_f^2,m_{f^\prime}^2)-B_0(0,m_f^2,m_{f^\prime}^2\Big)\Big]
 \quad\quad\quad\quad\: ....\:({\text{dia. r}})\nonumber\\
 \end{align}
 %
 \newpage
   \subsubsection{Higgs boson self energy :}
 \label{equ_ren_self_ww}  
   \begin{figure}[h!]
 \begin{center}
\includegraphics [angle=0,width=0.7\linewidth]{./one_loop/figures/h_h_self.eps}\\
	\caption{$\gamma{\text{-}Z}$ boson self energy diagrams at one loop.}
	\label{fig_ren_self_ww}
	\end{center}
\end{figure}
%
% 
 \begin{align}
 \Sigma^{H}(p^2)=&\quad\frac{3M_H^2}{8s_W^2M_W^2}\:A_0(M_H^2)\quad\quad\quad\quad\quad\quad\quad\quad\quad\quad\quad\quad\quad
 \quad\quad\quad\:\:
 ....\:({\text{dia. a}})\nonumber\\
 &+\frac{M_H^2}{8s_W^2M_W^2}\:A_0(M_Z^2)\quad\quad\quad\quad\quad\quad\quad\quad\quad\quad\quad\quad\quad
 \quad\quad\quad\: ....\:({\text{dia. b}})\nonumber\\
 &+\frac{M_H^2}{4s_W^2M_W^2}\:A_0(M_W^2)\quad\quad\quad\quad\quad\quad\quad\quad\quad\quad\quad\quad
 \quad\quad\quad\quad ....\: ({\text{dia. c}})\nonumber\\
 &+\frac{M_H^2}{4s_W^2c_W^2M_W^2}\:(4A_0(M_Z^2)-2M_Z^2C_I^R)\quad\quad\quad\quad\quad\quad\quad
 \quad\quad.... \:({\text{dia. d}})\nonumber\\
 &+\frac{1}{2s_W^2}\:(4A_0(M_W^2)-2M_W^2C_I^R)\quad\quad\quad\quad\quad\quad\quad\quad\quad\quad\quad
 \:\:\: .... \:({\text{dia. e}})\nonumber\\
 &+\frac{9M_H^4}{8s_W^2M_W^2}\:B_{0}(p^2,M_H^2,M_H^2)\quad\quad\quad\quad\quad\quad\quad\quad\quad\quad\quad
 \quad\:\:\:\: .... \:({\text{dia. f}})\nonumber\\
 &+\frac{M_H^4}{8s_W^2M_W^2}\:B_{0}(p^2,M_Z^2,M_Z^2)\quad\quad\quad\quad\quad\quad\quad\quad\quad\quad\quad
 \quad\quad .... \:({\text{dia. g}})\nonumber\\
  &+\frac{M_H^4}{4s_W^2M_W^2}\:B_{0}(p^2,M_W^2,M_W^2)\quad\quad\quad\quad\quad\quad\quad\quad\quad\quad\quad
 \quad\:\: .... \:({\text{dia. h}})\nonumber\\
 &-\frac{M_Z^2}{4s_W^2c_W^2}\:B_{0}(p^2,M_Z^2,M_Z^2)\quad\quad\quad\quad\quad\quad\quad\quad\quad\quad\quad
 \quad\quad\:\: .... \:({\text{dia. i}})\nonumber\\
  &-2\times\frac{M_W^2}{4s_W^2}\:B_{0}(p^2,M_W^2,M_W^2)\quad\quad\quad\quad\quad\quad\quad\quad
  \quad\quad
 \quad\quad\:\:\: .... \:({\text{dia. j and k}})\nonumber\\
 &-\frac{1}{4s_W^2c_W^2}\:\Big(2p^2B_{0}(p^2,M_Z^2,M_Z^2)+A_0(M_Z^2)\nonumber\\
 &\quad\quad\quad\quad +M_Z^2B_{0}(p^2,M_Z^2,M_Z^2)\Big)\quad\quad\quad\quad\quad\quad\quad
 \quad\quad\quad\:\:\:\:\: .... \:({\text{dia. l}})\nonumber\\
 &-2\times \frac{1}{4s_W^2}\:\Big(2p^2B_{0}(p^2,M_W^2,M_W^2)+A_0(M_W^2)\nonumber\\
 &\quad\quad\quad\quad +M_W^2B_{0}(p^2,M_W^2,M_W^2)\Big)\quad\quad\quad\quad\quad\quad\quad
 \quad\quad\quad\:\: .... \:({\text{dia. m and n}})\nonumber\\
 &+\frac{M_Z^2}{2s_W^2c_W^2}\:\Big(4B_0(p^2,M_Z^2,M_Z^2)-2C_I^R\Big)\quad\quad\quad\quad\quad\quad\quad
 \quad\quad .... \:({\text{dia. o}})\nonumber\\
 &+\frac{M_W^2}{s_W^2}\:\Big(4B_0(p^2,M_W^2,M_W^2)-2C_I^R\Big)\quad\quad\quad\quad\quad\quad\quad
 \quad\quad\quad .... \:({\text{dia. p}})\nonumber\\
 &-\frac{N_cm_f^2}{2s_W^2M_W^2}\Big[2A_0(m_f^2)+(4m_f^2-p^2)B_0(p^2,m_f^2,m_f^2)\Big]
 \quad\quad\quad\:\: ....\:({\text{dia. q}})\nonumber\\
 \end{align}
 %
 \newpage
 \subsubsection{Fermion self energy :}
 \label{equ_ren_self_fermion}  
   \begin{figure}[h!]
 \begin{center}
\includegraphics [angle=0,width=0.7\linewidth]{./one_loop/figures/fermion_self.eps}\\
	\caption{$\gamma{\text{-}Z}$ boson self energy diagrams at one loop.}
	\label{fig_ren_self_ww}
	\end{center}
\end{figure}
%
\begin{align}
 \Sigma^{f}(p^2)=&-\frac{m_f^2}{4s_W^2M_W^2}\:\delta_{ij}\:
 \Big[\slashed{p}LB_1(p^2,m_f^2,M_H^2)\nonumber\\
 &\quad\quad \slashed{p}RB_1(p^2,m_f^2,M_H^2)-m_fB_0(p^2,m_f^2,m_H^2)\Big]
 \quad\quad\quad\quad....\:({\text{dia. a}})\nonumber\\
 &-\quad\frac{m_f^2}{4s_W^2M_W^2}\:\delta_{ij}\:
 \Big[-\slashed{p}LB_1(p^2,m_f^2,M_Z^2)\nonumber\\
 &\quad\quad-\slashed{p}RB_1(p^2,m_f^2,M_Z^2)-m_fB_0(p^2,m_f^2,M_Z^2)\Big]
 \quad\quad\quad\quad....\:({\text{dia. b}})\nonumber\\
 &-\quad\frac{m_f^2}{2s_W^2M_W^2}\:\sum_k V_{ik}V^{*}_{kj}\:
 \Big[\slashed{p}\Big(L\:m_{f^\prime,k}^2+R\:m_{f,i}\:m_{f,j})B_1(p^2\nonumber\\
 &\quad\quad\quad ,m_{f^\prime,k}^2,M_W^2)+m_{f^\prime,k}^2B_0(p^2,m_{f^\prime,k}^2,M_W^2)(m_{f,i}L+m_{f,j}R)\Big]
....\:({\text{dia. c}})\nonumber\\
&-Q_f^2\:\delta_{ij}\:
 \Big[\slashed{p}L(2B_1(p^2,m_f^2,0)+C_I^R)\nonumber\\
 &\quad\quad\quad \slashed{p}R(2B_1(p^2,m_f^2,0)+C_I^R)+2m_f(2B_0(p^2,m_f^2,0)-C_I^R)\Big]
 \quad\quad\quad\quad....\:({\text{dia. d}})\nonumber\\
 &-\:\delta_{ij}\:
 \Big[\slashed{p}(g_f^-)^2L(2B_1(p^2,m_f^2,M_Z^2)+C_I^R)+ \slashed{p}(g_f^+)^2R(2B_1(p^2,m_f^2,M_Z^2)\nonumber\\
 &\quad\quad\quad +C_I^R)+g_f^- g_f^+ m_f(4B_0(p^2,m_f^2,M_Z^2)-C_I^R)\Big]
 \quad\quad\quad\quad\quad\quad....\:({\text{dia. e}})\nonumber\\
 &-\quad\frac{1}{2s_W^2}\:\sum_k V_{ik}V^{*}_{kj}\:
 \slashed{p}L\Big(2B_1(p^2,m_{f^\prime,k}^2,M_W^2)+C_I^R)\Big)
\quad\quad\quad\quad....\:({\text{dia. f}})\nonumber\\
\end{align}
 %
 \newpage
 \subsection{Counterterms}
 \label{equ_ren_ct_dia_ew}  
   \begin{figure}[h!]
 \begin{center}
\includegraphics [angle=0,width=0.8\linewidth]{./one_loop/figures/ct_dia_ew.eps}\\
	\caption{Counterterms for self energy and vertex diagrams.}
	\label{fig_ren_ct_dia_ew}
	\end{center}
\end{figure}
%
\begin{align}
{\text{Dia. a : }} CT_{ZZ}\equiv -ig^{\mu\nu}\Big[\delta Z_{ZZ}
\end{align}
 %

==> summary/summary.tex <==
\chapter*{Summary}
%\section{dd}
\label{chap_summery}
%\minitoc
  In the present day, the standard model is known for its illustrious success in describing the fundamental building blocks of nature. Despite its great success, the standard model has a few limitations in describing nature fully. 
  This motivates physicists to consider beyond-the-standard model scenarios, which may address the limitations of the standard model. Despite the elegance of some of the beyond-the-standard model theories, no significant departure from the standard model predictions has been found in colliders at current energy scales.
  After the discovery of the Higgs boson at the Large Hadron Collider, its properties have been studied extensively. They are found to be consistent with the standard model.
  However, some of the Higgs boson couplings are still not well determined. Self-couplings of the Higgs boson and the couplings with  some of the standard model particles still do not have stringent bounds.
  
  In this thesis, our main focus is on the $HHH$ and $VVHH$ couplings which are loosely bound. The $HHH$ coupling will determine the shape the Higgs potential and $VVHH$ couplings will tell us how the gauge bosons are coupled to the Higgs fields. We consider a few processes of Higgs boson production and decay to study these couplings.
   We investigate these processes in the context of the $\kappa$-framework to study the anomalous behavior of $HHH$ and $VVHH$ couplings. We calculate one-loop QCD and electroweak correction for these processes.
   In this thesis, we discuss spinor helicity formalism, which has been used in computing Feynman amplitudes for QCD and electroweak correction to these processes. We discuss one-loop Feynman integrals and one-loop electroweak renormalization in this thesis.
    We compute all possible self-energy contributions at one-loop for electroweak renormalization. We adopt Catani-Saymour dipole subtraction technique to have IR-safe amplitudes.
    
    In this thesis, in the first work, we consider the process $b\bar{b}\rightarrow W^+W^-H$. Due to the non-negligible coupling of the Higgs boson with the bottom quarks, there is a dependence on the $WWHH$ coupling in this process.
    This process receives the largest contribution when the W bosons are longitudinally polarized. We compute one-loop QCD corrections to various ﬁnal states with polarized $W$ bosons. We ﬁnd that the corrections to the ﬁnal state with the longitudinally polarized $W$ bosons are large.
     It is shown that the measurement of the polarization of the W bosons can be used as a tool to probe the $WWHH$ coupling in this process. We also examine the effect of varying $WWHH$ coupling in the $\kappa$-framework. The variation in the cross-section is significantly high when we consider longitudinally polarized $W$ bosons.
     In the second work, we study one-loop electroweak correction to $H\rightarrow \nu_e\bar{\nu_e}\nu_\mu\bar{\nu_\mu}$. 
     We discuss $\gamma^5$-anomaly, complex mass scheme and input parameter schemes which are relevant for one-loop electroweak correction.
     The corrections depend on the $HHH$ and $ZZHH$ couplings. We investigate this dependence in $\kappa$-framework. We find that the width depends on $HHH$ coupling significantly.
      The dependence on $ZZHH$ coupling is marginal in the $\alpha(M_Z)$ scheme but significant in the $G_F$ scheme. We also study the dependence on $ZZW W$ coupling. The scaling of $HHH$ coupling does not violate gauge invariance but the scaling of $ZZHH$ and $ZZWW$ couplings violate gauge invariance.
      In the third work, we study one-loop electroweak correction to the $H\rightarrow e^+e^-\mu^+\mu^-$ process. The corrections depend on $HHH$ and $ZZHH$ couplings.
      This process has IR divergences which we handle by adopting Catani-Saymour dipole subtraction for QED.
      We observe the same behavior in the relative change of the decay width for this process as the process $H\rightarrow \nu_e\bar{\nu_e}\nu_\mu\bar{\nu_\mu}$ when we vary $HHH$ and $ZZHH$ couplings.
  
  
  

 
